Benchmarking Domain Adaptation for Chemical Processes on the Tennessee Eastman Process

In system monitoring, automatic fault diagnosis seeks to infer the systems' state based on sensor readings, e.g., through machine learning models. In this context, it is of key importance that, based on historical data, these systems are able to generalize to incoming data. In parallel, many factors may induce changes in the data probability distribution, hindering the possibility of such models to generalize. In this sense, domain adaptation is an important framework for adapting models to different probability distributions. In this paper, we propose a new benchmark, based on the Tennessee Eastman Process of Downs and Vogel (1993), for benchmarking domain adaptation methods in the context of chemical processes. Besides describing the process, and its relevance for domain adaptation, we describe a series of data processing steps for reproducing our benchmark. We then test 11 domain adaptation strategies on this novel benchmark, showing that optimal transport-based techniques outperform other strategies.

==> content/tmp_da_methods.tex <==
Starting with single-source \gls{da}, \gls{tca} was first introduced by~\cite{pan2010domain}, and consists in projecting data onto a subspace where the \gls{mmd} between domains is minimal. Let $\mathbf{K}$ be the kernel matrix, defined as,
\begin{equation*}
    \mathbf{K} = \begin{bmatrix}
        \mathbf{K}_{SS} & \mathbf{K}_{ST}\\
        \mathbf{K}_{TS} & \mathbf{K}_{TT}
    \end{bmatrix}
\end{equation*}
\gls{tca} is based on the following optimization problem,
\begin{eqnarray*}
	\mathbf{W}^{\star} = &\underset{\mathbf{W}}{\text{minimize}}& \text{Tr}(\mathbf{W}^{T}\mathbf{W}) + \mu\text{Tr}(\mathbf{W}^{T}\mathbf{KLKW})\\
	&\text{subject to}& \mathbf{W}^{T}\mathbf{KHKW} = \mathbf{I}_{n}\nonumber
\end{eqnarray*}
where $\mathbf{W}^{\star} \in \mathbb{R}^{n_{f} \times n_{f}'}$, $\mathbf{H} = \mathbf{I}_{n} - \nicefrac{1}{n}\mathds{1}_{n}\mathds{1}_{n}^{T}$ is the centering matrix, and $\mu > 0$ is the penalty coefficient. The projection matrix $\mathbf{W}^{\star}$ can be used for mapping points into $\mathbb{R}^{n_{f}'}$, through $T(\mathbf{X}) = \mathbf{K}\mathbf{W}^{\star}$.

\gls{otda}~\cite{courty2016otda} consists on matching $\hat{P}_{S}$ and $\hat{P}_{T}$ through \gls{ot}. The approach relies on the notion of barycentric mapping, defined as,
\begin{align}
    T_{\gamma}(\mathbf{x}_{i}^{(P_{S})}) = n_{S}\gamma^{\star}\mathbf{X}^{(P_{T})},\label{eq:barymap},
\end{align}
where $\gamma^{\star}$ is the \gls{ot} plan between $\hat{P}_{S}$ and $\hat{P}_{T}$.

Next, deep \gls{da} methods reduce the distance in distribution between $\phi_{\sharp}\hat{Q}_{S}$ and $\phi_{\sharp}\hat{Q}_{T}$ through a domain dissimilarity loss $\mathcal{L}_{d}$, that is:
\begin{equation*}
    (\theta_{\phi}^{\star}, \theta_{h}^{\star}) = \min{\theta_{\phi}, \theta_{h}}\hat{\mathcal{R}}_{S}(h \circ \phi) + \lambda \mathcal{L}_{d}(\theta_{\phi}, \theta_{h}),
\end{equation*}
where $\theta_{\phi}$ and $\theta_{h}$ are the parameters (i.e., weights) of $\phi$ and $h$ respectively. In this context, \cite{ghifary2014domain} introduced a method that relies on minimizing the \gls{mmd} between features distributions,
\begin{align*}
    \mathcal{L}_{d}(\theta_{\phi}) = \text{MMD}_{k}(\phi_{\sharp}\hat{Q}_{S},\phi_{\sharp}\hat{Q}_{T})^{2}.
\end{align*}
henceforth we refer to this method as \gls{mmd}. \gls{dann} was proposed by~\cite{ganin2016domain}, and relies on the $\mathcal{H}-$distance. The authors propose an additional domain classifier branch, $h_{d}$. The domain loss term thus corresponds to,
\begin{align*}
    \mathcal{L}_{d}(\theta_{\phi}) &= \max{\theta_{h_{d}}}\dfrac{1}{n}\sum_{i=1}^{n}\log(1 - h_{d}(\phi(\mathbf{x}_{i}^{(Q_{S})}))) + \dfrac{1}{m}\sum_{i=1}^{m}\log(h_{d}(\phi(\mathbf{x}_{j}^{(Q_{T})}))).
\end{align*}
In other words, $\phi$ is trained so as to \emph{maximize} domain confusion.

We further discuss the \gls{jdot} method of~\cite{courty2017joint}, and its latter deep \gls{da} extension proposed by~\cite{damodaran2018deepjdot}. This strategy models feature-label joint distributions, but, since the target domain is not labeled, one uses the approximation,
\begin{align*}
    \hat{Q}_{T}^{h}(\mathbf{x},y) &= \dfrac{1}{n_{T}}\sum_{j=1}^{n_{T}}\delta((\mathbf{x},y) - (\mathbf{x}_{i}^{(Q_{T})}, h(\mathbf{x}_{i}^{(Q_{T})}))),
\end{align*}
which serves as a proxy for $\hat{Q}_{T}(\mathbf{x},\mathbf{y})$. The idea of~\cite{courty2017joint} is minimizing $W_{2}(\hat{Q}_{S}, \hat{Q}_{T}^{h})$ with ground cost,
\begin{align}
    C_{ij} &= \alpha\lVert \mathbf{x}_{i}^{(Q_{S})} - \mathbf{x}_{j}^{(Q_{T})}\rVert_{2}^{2} + \beta \mathcal{L}_{c}(y_{i}^{(Q_{S})}, h(\mathbf{x}_{j}^{(Q_{T})})).\label{eq:jdot_gcost}
\end{align}
The \gls{jdot} strategy thus minimizes,
\begin{align*}
\min{h\in\mathcal{H},\gamma\in\Gamma(\hat{Q}_{S},\hat{Q}_{T}^{h})}\sum_{i=1}^{n_{S}}\sum_{j=1}^{n_{T}}\gamma_{ij}C_{ij} = \min{h\in\mathcal{H}}W_{2}(\hat{Q}_{S}, \hat{Q}_{T}^{h})^{2},
\end{align*}
by alternating the minimization over $h$ and $\gamma$. As follows,~\cite{damodaran2018deepjdot} extended the \gls{jdot} framework for deep \gls{da}, by defining $\mathcal{L}_{d}(\theta_{\phi})$ as,
\begin{align*}
\min{\gamma\in\Gamma(\hat{Q}_{S},\hat{Q}_{T}),h}\sum_{i=1}^{n_{S}}\sum_{j=1}^{n_{T}}\gamma_{i,j}(\alpha\lVert \phi(\mathbf{x}_{i}^{(Q_{S})}) - \phi(\mathbf{x}_{j}^{(Q_{T})})\rVert_{2}^{2} + \beta \mathcal{L}_{c}(y_{i}^{(Q_{S})}, h(\mathbf{x}_{j}^{(Q_{T})}))),
\end{align*}
as domain dissimilarity.

Now, for multi-source \gls{da}, \gls{wbt}, proposed by~\cite{montesuma2021icassp,montesuma2021cvpr}, is a method that relies on the Wasserstein barycenter for aggregating source distributions before transferring to target. Therefore, the authors propose solving,
\begin{align}
    \mathcal{B}(\alpha;\mathcal{P}) &= \argmin{\substack{\mathbf{x}^{(B)}_{1},\cdots,\mathbf{x}^{(B)}_{j},\cdots,\mathbf{x}^{(B)}_{n} \in \mathbb{R}^{d}\\ \mathbf{y}^{(B)}_{1},\cdots,\mathbf{y}^{(B)}_{j},\cdots,\mathbf{y}^{(B)}_{n} \in \mathbb{R}^{d}}}\sum_{\ell=1}^{N}\alpha_{\ell}\langle \gamma^{(\ell)}, \mathbf{C}^{(\ell)} \rangle_{F},\label{eq:wbary}\\
    C_{ij}^{(k)} &= \lVert \mathbf{x}_{i}^{(P_{S_{\ell}})}-\mathbf{x}_{j}^{(B)} \rVert_{2}^{2} + \beta \delta(\mathbf{y}_{i}^{(P_{S_{\ell}})} -\mathbf{y}_{j}^{(B)}),\label{eq:supervised_gcost}
\end{align}
for $\alpha_{k}=\nicefrac{1}{N}$, and $\beta > 0$ corresponding to how costly it is to transport points from different classes. This minimization problem is carried out by iterating,
\begin{equation*}
    \mathbf{X}^{(B)}_{it+1} = \sum_{\ell=1}^{N}\alpha_{\ell}T_{\gamma^{(\ell)}}(\mathbf{X}^{(B)}_{it}),\text{ and }\mathbf{Y}^{(B)}_{it+1} = \sum_{\ell=1}^{N}\alpha_{\ell}T_{\gamma^{(\ell)}}(\mathbf{Y}^{(B)}_{it}),
\end{equation*}
until convergence. For \gls{da}, the empirical distribution $\hat{B}$ with support $\{(\mathbf{x}_{i}^{(B)}, \mathbf{y}^{(B)}_{i})\}_{i=1}^{n_{B}}$ represents an intermediate domain. As follows,~\cite{montesuma2021icassp,montesuma2021cvpr} employ an additional step for transporting $\hat{B}$ towards $\hat{P}_{T}$, through the barycentric mapping, i.e. $T_{\gamma}(\mathbf{X}^{(B)})$ (see equation~\ref{eq:barymap}).

\gls{dadil} was proposed by~\cite{montesuma2023learning}, and consists on learning a dictionary over source domain distributions. The dictionary is a pair $(\mathcal{Q}, \mathcal{A})$, of a set of atoms $\mathcal{Q}=\{\hat{Q}_{k}\}_{k=1}^{K}$ and weights $\mathcal{A} = \{\alpha_{\ell}\}_{\ell=1}^{N+1}$, where $\alpha_{\ell}$ are the barycentric coordinates of $\hat{P}_{\ell}$ w.r.t. $\mathcal{Q}$. By convention, the authors use $\alpha_{N+1} = \alpha_{T}$.

Each atom is parametrized by its support, that is, $\hat{Q}_{k}=\dfrac{1}{n}\sum_{i=1}^{n}\delta_{(\mathbf{x}_{i}^{(Q_{k})},\mathbf{y}_{i}^{(Q_{k})})}$. The dictionary learning setting consists on a minimization problem,
\begin{align*}
    (\mathcal{Q}^{\star},\mathcal{A}^{\star}) = \argmin{\mathcal{Q},\mathcal{A}\in\Delta_{K}^{N+1}}\dfrac{1}{N+1}\sum_{\ell=1}^{N+1}W_{c}(\hat{P}_{\ell},\mathcal{B}(\alpha_{\ell};\mathcal{Q})),
\end{align*}
where $W_{c}$ is the Wasserstein distance with,
\begin{align*}
    C_{ij} &= \lVert \mathbf{x}_{i}^{(P)}-\mathbf{x}_{j}^{(Q)} \rVert_{2}^{2} + \beta \lVert \mathbf{y}_{i}^{(P)} -\mathbf{y}_{j}^{(Q)} \rVert^{2},
\end{align*}
Since the target $\hat{P}_{T}$ is not labeled, one cannot compute $W_{c}(\hat{P}_{T}, \hat{B}_{T})$ directly. We use \gls{ot} for pseudo-labeling the target domain, that is,
\begin{align*}
    \hat{\mathbf{Y}}^{(P_{T})} = \dfrac{1}{N_{S}}\sum_{\ell=1}^{N_{S}}n_{\ell}(\pi_{\ell})^{T}\mathbf{Y}^{(P_{\ell})},
\end{align*}
where $\pi_{\ell} = \text{OT}(\mathbf{X}^{(P_{\ell})}, \mathbf{X}^{(P_{T})})$. We illustrate the overall idea behind \gls{dadil} in figure~\ref{fig:dadil}.

Once the dictionary is learned, the authors propose two methods for \gls{msda}. The first, called \gls{dadil}-R, is based on the reconstruction $\hat{B}_{T} = \mathcal{B}(\alpha_{T};\mathcal{Q})$:
\begin{equation*}
\mathbf{X}^{(B_{T})} = \sum_{k=1}^{K}\alpha_{k}T_{\gamma^{(k)}}(\mathbf{X}^{(Q_{k})})\text{, }\mathbf{Y}^{(B_{T})} = \sum_{k=1}^{K}\alpha_{k}T_{\gamma^{(k)}}(\mathbf{Y}^{(Q_{k})}),\\
\end{equation*}
which allows to reconstruct labeled samples in a distribution close to $\hat{P}_{T}$. The second method, called \gls{dadil}-E, exploits the fact that each $\hat{Q}_{k}$ is labeled, for learning an \emph{atomic classifier}, i.e. $\hat{h}_{k} = \text{argmin}_{h\in\mathcal{H}}\hat{\mathcal{R}}_{Q_{k}}(h)$. For predicting samples on $\hat{P}_{T}$, \gls{dadil}-E weights the predictions of the various atomic classifiers, i.e.,
\begin{align*}
    \hat{h}_{\alpha_{T}}(\mathbf{x}_{j}^{(P_{T})}) = \sum_{k=1}^{K}\alpha_{T,k}\hat{h}_{k}(\mathbf{x}_{j}^{(P_{T})}).
\end{align*}
The intuition for this method is twofold. First, if $\hat{Q}_{k}$ is close in distribution to $\hat{P}_{T}$, it is likely to yield a good predictor for the target domain. Second, the close $\hat{Q}_{k}$ and $\hat{P}_{T}$ are, the higher will be the weights $\alpha_{T,k}$, so its predictions become more important.

\gls{m3sda}, proposed by~\cite{peng2019moment}, employs an architecture based on a shared encoder $\phi$, and $N$ domain-specific classifiers, i.e, $\{h_{k}\}_{n=1}^{N}$. Their architecture couples the \gls{erm} procedure with a regularization term based on the moments of domains $k=1,\cdots,N$,
\begin{align*}
    \mathcal{L}_{d}(\phi) &= \Omega_{S}(\phi) + \Omega_{T}(\phi),\\
    \Omega_{S}(\phi) &= \dfrac{1}{N}\sum_{p=1}^{2}\sum_{i=1}^{N}\lVert \mu_{S_{i}}^{p} - \mu_{T}^{p}  \rVert_{2},\\
    \Omega_{T}(\phi) &= \binom{N}{2}\sum_{p=1}^{2}\sum_{i=1}^{N-1}\sum_{j=i+1}^{N}\lVert \mu_{S_{i}}^{p}-\mu_{S_{j}}^{p} \rVert_{2}.
\end{align*}
where $\mu_{S_{i}}^{p}=\mathbb{E}_{\mathbf{x}\sim P_{S_{i}}}[\phi(\mathbf{x})^{p}]$ corresponds to the entry-wise power of the mean vector on the $i-$th source (resp. target). This is similar to a \gls{mmd} distance between sources $i$ and $j$, and each source and the target, for a polynomial kernel. The \gls{m3sda} algorithm is based on the optimization problem,
\begin{align}
    \min{\phi,\{h_{k}\}_{k=1}^{N}}\dfrac{1}{N}\sum_{k=1}^{N}\hat{\mathcal{R}}_{S_{\ell}}(h_{k}\circ \phi) + \Omega(\phi).\label{eq:m3sda}
\end{align}
\cite{peng2019moment} further proposes \gls{m3sda}-$\beta$, which employs pairs of classifiers $\{(h_{k},h_{k}')\}_{k=1}^{K}$. Besides minimizing~\ref{eq:m3sda}, they add other 2 learning phases. First,
\begin{align*}
    \min{h'_{k}}\sum_{k=1}^{N}\hat{\mathcal{R}}_{S_{\ell}}(h_{k}' \circ \phi) - \sum_{k=1}^{N}\sum_{j=1}^{n_{T}}|h_{k}(\mathbf{z}_{j}^{(P_{T})})-h_{k}'(\mathbf{z}_{j}^{(P_{T})})|,
\end{align*}
where the second term denotes the output discrepancy on the target domain of $(h_{k},h_{k}')$. Second,
\begin{align*}
    \min{\phi} \sum_{k=1}^{N}\sum_{j=1}^{n_{T}}|h_{k}(\phi(\mathbf{x}_{j}^{(P_{T})}))-h_{k}'(\phi(\mathbf{x}_{j}^{(P_{T})}))|.
\end{align*}
Thus, \gls{msda}-$\beta$ consists on alternating between the three training steps at each iteration. For generating the final predictions on the target domain,~\cite{peng2019moment} proposes weighting the domain-specific classifiers predictions, i.e.,
\begin{align*}
    \hat{y}^{(P_{T})} = \sum_{k=1}^{N}w_{k}h_{k}(\mathbf{x}^{(P_{T})}),
\end{align*}
for $w_{k} = acc_{k}/\sum_{\ell=1}^{N}acc_{\ell}$, where $acc_{k}$ denotes the classification accuracy of $h_{k}$ on its respective domain. The overall architecture of these 2 methods is shown in figure~\ref{fig:m3sda}.

\gls{wjdot}, proposed by~\cite{turrisi2022multi}, adapts the \gls{jdot} framework for \gls{msda}. Given $\alpha \in \Delta_{N}$, the authors aggregate $\{\hat{P}_{S_{\ell}}\}_{k=1}^{N}$ linearly, namely,
\begin{align*}
    \hat{P}_{\alpha} &= \sum_{k=1}^{N}\alpha_{k}\hat{P}_{k} = \sum_{k=1}^{N}\dfrac{\alpha_{k}}{n_{S_{\ell}}}\sum_{i=1}^{n_{S_{\ell}}}\delta_{(\mathbf{x}^{(P_{S_{\ell}})},y^{(P_{S_{\ell}})})},
\end{align*}
that is, $\hat{P}_{\alpha}$ is a distribution with $n = \sum_{k}n_{S_{\ell}}$ samples, with different importance (i.e. $\alpha_{k}/n_{S_{\ell}}$). \gls{wjdot} then minimizes,
\begin{align*}
    \argmin{\alpha \in \Delta, h \in \mathcal{H}}W_{c}(\hat{P}_{\alpha}, \hat{P}_{T}^{h}),
\end{align*}
which is carried, as in~\gls{jdot}, by alternating between minimizing $\alpha$ for fixed $h \in \mathcal{H}$ and vice-versa.

==> content/tmp_preliminaries.tex <==
\section{Preliminaries}\label{sec:preliminaries}

\subsection{Learning Theory}

In machine learning, classification can be formalized under the \gls{erm} framework~\cite{vapnik2013nature}. Let $\mathcal{H}$ be a family of functions from a feature space $\mathcal{X}$ (e.g., $\mathbb{R}^{d}$) to a label space $\mathcal{Y}$ (e.g., $\{1,\cdots,n_{c}\}$). Let $P \in \mathbb{P}(\mathcal{X})$ be a probability distribution, $h_{0}$ be a ground-truth labeling function, and $\mathcal{L}$ be a loss function. The \gls{erm} framework revolves around the idea of risk of a classifier $h \in \mathcal{H}$,
\begin{align*}
    \mathcal{R}_{P}(h) = \expectation{\mathbf{x} \sim P}[\mathcal{L}(h(\mathbf{x}), h_{0}(\mathbf{x}))] = \int_{\mathcal{X}}\mathcal{L}(h(\mathbf{x}), h_{0}(\mathbf{x}))dP(\mathbf{x}).
\end{align*}
$\mathcal{R}_{P}$ can be interpreted as the error rate of $h$. Based on this idea, it is natural to choose $h^{\star} = \text{argmin}_{h\in\mathcal{H}}\mathcal{R}_{P}(h)$. In practice, $P$ and $h_{0}$ are not known a priori. Indeed, one rather has access to samples $\{(\mathbf{x}_{i}^{(P)}, y_{i}^{(P)})\}_{i=1}^{n}$, where $\mathbf{x}_{i}^{(P)} \iid P$ and $y_{i}^{(P)} = h_{0}(\mathbf{x}_{i}^{(P)})$. These ideas lead to the notion of empirical risk,
\begin{definition}{(Empirical Risk)}
    Let $\{(\mathbf{x}_{i}^{(P)}, y_{i}^{(P)})\}_{i=1}^{n}$ be a dataset, and $\mathcal{L}$ be a loss function. The empirical risk of $h \in \mathcal{H}$ is,
    \begin{align}
        \hat{\mathcal{R}}_{P}(h) = \dfrac{1}{n}\sum_{i=1}^{n}\mathcal{L}(h(\mathbf{x}_{i}^{(P)}),y_{i}^{(P)}).\label{eq:emp_risk}
    \end{align}
    Furthermore, a classifier $\hat{h}$ is said to fit the data if $\hat{h} = \text{argmin}_{h \in \mathcal{H}}\hat{\mathcal{R}}_{P}(h)$.
\end{definition}

As a consequence, the \gls{erm} turns the learning problem into an optimization problem. One may further note that, in practice, one estimates $\hat{h}$ by parametrizing classifiers. For instance, one may have linear classifiers, in which case $\mathcal{H} = \{h(\mathbf{x}) = \mathbf{Ax} + \mathbf{b} : \mathbf{A} \in \mathbb{R}^{d \times n_{c}}, \mathbf{b} \in \mathbb{R}^{n_{c}}\}$. In this paper, we consider deep neural nets composed of 2 parts: an encoder network $\phi$, and a classifier $h$. The encoder maps data $\mathbf{x} \in \mathcal{X}$ into a latent representation $\mathbf{z} \in \mathcal{Z}$, whereas the classifier maps the representation into a label space $\mathcal{Y}$.

\begin{figure}[ht]
    \centering
    \includegraphics[width=0.7\linewidth]{Figures/deep_nn_en.pdf}
    \caption{\textbf{Illustration of a deep neural net,} where data $\mathbf{x}_{i}^{(P)}$ are mapped into latent representation vectors $\mathbf{z}_{i}^{(P)}$ through an encoder $\phi$. The latent representation is then used to predict a class, i.e., $\hat{y}_{i}^{(P)}$.}
    \label{fig:deep_nn}
\end{figure}

In the context of the presented concepts, we may further make a parallel between classification and \gls{afd} systems. In the latter case, one seeks to determine which fault has occurred, based on sensor readings. As such, one may identify $\mathcal{X} = \mathbb{R}^{d \times T}$ as the space of time series, for $d$ distributionments over $T$ time steps. The \gls{afd} system then produces a diagnostic, which can be a probability vector $\hat{\mathbf{y}}_{i}^{(P)} \in \Delta_{n_{c}}$, or a categorical value $y_{i}^{(P)} \in \{1,\cdots,n_{c}\}$.

\subsection{Principles of Domain Adaptation}\label{sec:da_principles}

\gls{da} is a field within transfer learning~\cite{pan2010domain}, where one seeks to improve performance on a target domain based on knowledge available in a source domain. In the following, we formalize these ideas.
\begin{definition}{(Transfer Learning~\cite{pan2010domain})}
    Let $\mathcal{X}$ be a feature space, and $\mathcal{Y}$ be a target space. A domain is a pair $\mathcal{D}=(\mathcal{X},Q)$, where $Q \in \mathbb{P}(\mathcal{X})$. Likewise, a task is a pair $\mathcal{T}=(\mathcal{Y},h_{0})$, where $h_{0}:\mathcal{X}\rightarrow\mathcal{Y}$ is a ground-truth labeling function. Transfer learning is a learning problem where one wants to improve performance on a target $(\mathcal{D}_{T},\mathcal{T}_{T})$ based on knowledge from a source $(\mathcal{D}_{S},\mathcal{T}_{S})$
\end{definition}
Based on this definition, \gls{da} is a sub-problem within transfer learning, where one has a single task (i.e., $\mathcal{T}_{S} = \mathcal{T}_{T}$), and different, but related domains (i.e., $\mathcal{D}_{S} \neq \mathcal{D}_{T}$). In most cases, $\mathcal{X}$ is fixed, and one has different feature probability distributions (i.e., $Q_{S} \neq Q_{T}$).

In our experiments, we focus on methods that seek to minimize a distance between probability distributions through a data transformation $T$. This transformation can either map the original data into a new space, or simply transform the data in the same ambient space. Associated with $T$, there is the notion of pushforward mapping~\cite{peyre2019computational}, which creates a new distribution based on the action of $T$ on samples, that is, $T_{\sharp}\hat{Q}_{S} = \dfrac{1}{n}\sum_{i=1}^{n}\delta_{\mathbf{x}_{i}^{(Q_{S})}}$. The principle behind the methods we consider is to find a transformation that aligns $\hat{Q}_{S}$ and $\hat{Q}_{T}$, in a distribution space. As a result, a classifier learned on the transformed data is able to generalize to the target domain.
\begin{figure}[ht]
    \centering
    \includegraphics[width=0.7\linewidth]{Figures/illustration_domain_adaptation.pdf}
    \caption{\textbf{Domain adaptation based on data transformation.} In an ambient space, source and target data follow different probability distributions. As a result, a classifier learned on the source (blue straight line on the left) is not able to generalize on data from the target domain (orange elements). In this paper we consider methods that align the distributions through a data transformation $T$, which maps data into a latent space.}
    \label{fig:illustration_da}
\end{figure}

The alignment of probability distributions supposes a criterion of \emph{dissimilarity} between these objects. In this sense, one may use \emph{probability metrics}, which are distances in the space of probability distributions, i.e., $\mathbb{P}(\mathbb{R}^{d})$. Here, we consider three prominent metrics, namely, the $\mathcal{H}$-distance, the \gls{mmd} and the Wasserstein distance.

The $\mathcal{H}$-distance has its roots on \gls{da} theory~\cite{ben2010theory}. It measures the distance between distributions as how likely a classifier can separate samples from these distributions. Hence, let $h \in \mathcal{H}$ be a classifier,
\begin{align}
    d_{\mathcal{H}}(\hat{Q}_{S},\hat{Q}_{T}) = 2\biggr(1-\min{h\in\mathcal{H}}\dfrac{1}{n}\sum_{i=1}^{n}\log(1-h(\mathbf{x}_{i}^{(Q_{S})})) + \dfrac{1}{m}\sum_{j=1}^{m}\log h(\mathbf{x}_{j}^{(Q_{T})})\biggr).
\end{align}
Hence, the $d_{\mathcal{H}}$ can be easily estimated from samples $\{\mathbf{x}_{i}^{(Q_{S})}\}_{i=1}^{n}$ and $\{\mathbf{x}_{j}^{(Q_{T})}\}_{j=1}^{m}$. First, one artificially labels samples from $Q_{S}$ with a label $0$, and labels from $Q_{T}$ with a label $1$. Then, one learns a classifier to distinguish samples from $Q_{S}$ from those of $Q_{T}$ (e.g., through a \gls{svm} or a \gls{nn}).

The \gls{mmd} has its roots on kernel theory~\cite{gretton2007kernel}, and was initially proposed to test if two samples come from the same distribution. Let $k:\mathbb{R}^{d}\times\mathbb{R}^{d}\rightarrow\mathbb{R}$ be a kernel, the \gls{mmd} can be defined as,
\begin{equation}
\begin{aligned}
    \text{MMD}_{k}(\hat{Q}_{S},\hat{Q}_{T})^{2} = \dfrac{1}{n^{2}}\sum_{i=1}^{n}\sum_{j=1}^{n}k(\mathbf{x}_{i}^{(Q_{S})},\mathbf{x}_{j}^{(Q_{S})}) &+ \dfrac{1}{m^{2}}\sum_{i=1}^{m}\sum_{j=1}^{m}k(\mathbf{x}_{i}^{(Q_{T})},\mathbf{x}_{j}^{(Q_{T})})\\
    &- \dfrac{2}{nm}\sum_{i=1}^{n}\sum_{j=1}^{m}k(\mathbf{x}_{i}^{(Q_{S})},\mathbf{x}_{j}^{(Q_{T})}),
\end{aligned}
\end{equation}
examples of kernels include the linear kernel $k(\mathbf{x}_{i}^{(Q_{S})},\mathbf{x}_{j}^{(Q_{T})}) = (\mathbf{x}_{i}^{(Q_{S})})^{\top}\mathbf{x}_{j}^{(Q_{T})}$, and the Gaussian kernel, $k(\mathbf{x}_{i}^{(Q_{S})},\mathbf{x}_{i}^{(Q_{T})}) = \exp{(-\gamma\lVert \mathbf{x}_{i}^{(Q_{S})} - \mathbf{x}_{j}^{(Q_{T})} \rVert_{2}^{2})}$, for a parameter $\gamma > 0$. Intuitively, the \gls{mmd} is a distance between the means of distributions in an embedding space defined by the kernel $k$.

Finally, the Wasserstein distance $W_{p}$ is rooted on the theory of \gls{ot}. In its modern computational treatment \cite{peyre2019computational,montesuma2023recent}, the \gls{ot} problem can be phrased as,
\begin{equation}
\gamma^{\star} = \text{OT}(\mathbf{X}^{(Q_{S})}, \mathbf{X}^{(Q_{T})}) = \argmin{\gamma \in \Gamma(\hat{Q}_{S},\hat{Q}_{T})}  \langle \gamma, \mathbf{C}\rangle_{F},\label{eq:kantorovich}
\end{equation}
where $\gamma \in \mathbb{R}^{n\times m}$ is called \gls{ot} plan, $\mathbf{C} \in \mathbb{R}^{n \times m}$ is the ground-cost matrix with $C_{ij} = \lVert \mathbf{x}_{i}^{(Q_{S})} - \mathbf{x}_{j}^{(Q_{T})} \rVert_{2}^{p}$, and $\langle \cdot, \cdot \rangle_{F}$ is the Frobenius dot product. The set $\Gamma(\hat{Q}_{S},\hat{Q}_{T}) = \{\gamma\in\mathbb{R}^{n_{S}\times n_{T}}:\sum_{i=1}^{n_{S}}\gamma_{i,j}=\nicefrac{1}{n_{S}}\text{ and }\sum_{j=1}^{n_{T}}\gamma_{i,j}=\nicefrac{1}{n_{T}}\}$. Problem~\ref{eq:kantorovich} is a linear program, which can be solved exactly through the Simplex method~\cite{dantzig1955generalized}. Based on $\gamma^{\star}$, the Wasserstein distance is $W_{p}(\hat{Q}_{S}, \hat{Q}_{T}) = \langle \gamma^{\star}, \mathbf{C} \rangle_{F}^{p}$.

As a final remark, note that one may have different, heterogeneous sources of data. This implies that the source domain is composed of different distributions as well, i.e., $Q_{S_{1}}, \cdots, Q_{S_{N}}$. This problem is known in the literature as \gls{msda}. Besides considering the shift $Q_{S_{\ell}} \neq Q_{T}$, one must also consider the shift between different sources, i.e., $Q_{S_{\ell}} \neq Q_{S_{\ell'}}$ for $\ell \neq \ell'$.

\begin{wraptable}{r}{0.5\linewidth}

\end{wraptable} 
In the following, we cover a series of experiments with \gls{da} methods that implement ways of minimizing the distance between $\hat{Q}_{S}$ and $\hat{Q}_{T}$ through a transformation $T$ of data. We divide methods between shallow and deep \gls{da}. The first kind of methods perform adaptation based on extracted or engineered features. The second kind perform adaptation during the training of a deep \gls{nn}. This means that the data transformation is exactly the encoder network, $\phi$. These methods include a term in the \gls{nn} loss, accounting for the distance between distributions $\hat{Q}_{S}$ and $\hat{Q}_{T}$. Besides this category, we further divide methods with respect the distance they minimize, and whether they assume a single, or multiple source domains. We consider, in total, 11 methods, which are listed in table~\ref{tab:overview_da}. We refer readers to the original papers of these algorithms for further details on their implementation.

